AV Taris: Online Audio-Visual Speech Recognition

In recent years, Automatic Speech Recognition (ASR) technology has approached human-level performance on conversational speech under relatively clean listening conditions. In more demanding situations involving distant microphones, overlapped speech, background noise, or natural dialogue structures, the ASR error rate is at least an order of magnitude higher. The visual modality of speech carries the potential to partially overcome these challenges and contribute to the sub-tasks of speaker diarisation, voice activity detection, and the recovery of the place of articulation, and can compensate for up to 15dB of noise on average. This article develops AV Taris, a fully differentiable neural network model capable of decoding audio-visual speech in real time. We achieve this by connecting two recently proposed models for audio-visual speech integration and online speech recognition, namely AV Align and Taris. We evaluate AV Taris under the same conditions as AV Align and Taris on one of the largest publicly available audio-visual speech datasets, LRS2. Our results show that AV Taris is superior to the audio-only variant of Taris, demonstrating the utility of the visual modality to speech recognition within the real time decoding framework defined by Taris. Compared to an equivalent Transformer-based AV Align model that takes advantage of full sentences without meeting the real-time requirement, we report an absolute degradation of approximately 3% with AV Taris. As opposed to the more popular alternative for online speech recognition, namely the RNN Transducer, Taris offers a greatly simplified fully differentiable training pipeline. As a consequence, AV Taris has the potential to popularise the adoption of Audio-Visual Speech Recognition (AVSR) technology and overcome the inherent limitations of the audio modality in less optimal listening conditions.

==> 4.Intuition.tex <==
\section{Why learn to count words}
\label{s4:intuition}

Proper lexical segmentation of speech depends on context and semantics, as commonly illustrated by the example \emph{how to wreck a nice beach} sounding similar to \emph{how to recognise speech}. Thus, strategies incrementally scanning for hard boundaries~\citep{Li2019, Hou2020, Dong2019} are less suited to word units, prompting~\cite{Dong2019} to perform beam search on the entire sequence of sub-word tokens estimated from each segment. Instead, Taris has to develop intrinsic word counting mechanisms. One plausible strategy is to incrementally gather lexical evidence at the sub-word level, and learn to represent boundary-informative acoustic cues on a manifold where they can be accumulated.

We conjecture that learning the ability to count words facilitates the segmentation of speech into words, and we discuss below our intuition behind it.

In Figure~\ref{fig:word_segment} we illustrate the word counting sub-problem to be solved by the network. Starting in the bottom left corner, the network predicts scores for every audio frame in the sentence, and the cumulative sum is promoted to get as close as possible to the total word count, shown with a red circle. There is a very large number of paths that can be taken to reach the target count. However, when trained on large amounts of naturally distributed speech, we predict that Taris converges towards genuine word segmentation by having the cumulative sum cross all the intermediate word boundaries shown with yellow circles. In other words, the network may learn to self-normalise the accumulated probabilities for each word regardless of their length or cued structure.

We believe it suffices to train a system with the right amount of speech data, with the following intuition. As words appear in multiple contexts throughout a dataset, learning to count words may then have a normalisation effect on the fraction of $\Sigma \hat{w}$ allocated to each word in a sentence. Each word unit will approach a unitary mass allocation as its acoustic realisation is seen more often in multiple contexts. For the less frequent words, the correct allocation may happen by marginalisation if the sentences they appear in contain relatively more frequent words. Loosely speaking, it is the task of solving a system of linear equations where the variables are the partial sums corresponding to the acoustic frames between two consecutive estimated boundaries. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=1.0\linewidth]{./pics/ws_patterns/ws_praat.pdf}
    \caption{Illustration of the word counting problem. Given a spoken phrase \emph{something like a garden compost}, the network has to reach the correct word count 5 taking any path starting in the bottom left corner. The blue path allows an easy segmentation of speech into words. The green and dark orange paths are possible, but do not facilitate segmentation.}
    \label{fig:word_segment}
\end{figure}

Since we do not explicitly model the pauses between words, and the convergence towards the segmental behaviour is a mathematical conjecture without analytic proof for now, it is likely to observe deviations in practice on learnt solutions. However, Taris does not require a very strict approximation of word boundaries to function correctly. Instead, it is sufficient to just avoid frequent under- and over-segmentation, as it directly impacts the model's latency. 


==> 7.Conclusion.tex <==
\section{Conclusion}
